Differential privacy with partial knowledge

Differential privacy offers formal quantitative guarantees for algorithms over datasets, but it assumes attackers that know and can influence all but one record in the database. This assumption often vastly overapproximates the attackers' actual strength, resulting in unnecessarily poor utility. Recent work has made significant steps towards privacy in the presence of partial background knowledge, which can model a realistic attacker's uncertainty. Prior work, however, has definitional problems for correlated data and does not precisely characterize the underlying attacker model. We propose a practical criterion to prevent problems due to correlations, and we show how to characterize attackers with limited influence or only partial background knowledge over the dataset. We use these foundations to analyze practical scenarios: we significantly improve known results about the privacy of counting queries under partial knowledge, and we show that thresholding can provide formal guarantees against such weak attackers, even with little entropy in the data. These results allow us to draw novel links between k-anonymity and differential privacy under partial knowledge. Finally, we prove composition results on differential privacy with partial knowledge, which quantifies the privacy leakage of complex mechanisms. Our work provides a basis for formally quantifying the privacy of many widely-used mechanisms, e.g. publishing the result of surveys, elections or referendums, and releasing usage statistics of online services.

==> appendices.tex <==
%!TEX root = paper.tex

% \section{Summary of notations}\label{notationtable}
%
% \input{notationtable.tex}

% \TODOd{make sure the table isn't floating elsewhere on the page}


\section{Outliers under NP and DDP}\label{ex:outliers}

Consider the same $\theta$ as for Example~\ref{ex:cw}: it depends on a global
parameter, $\mu$, which is either +1 or -1 with equal probabilities, and each of
the $n$ records is normally distributed with mean $\mu$ and a small standard
deviation $\sigma$. Let $\mecha$ be the algorithm that counts \emph{outliers}:
it computes the average $\tilde{\mu}$ of all data points, and returns the number
of records outside $\left[\tilde{\mu}-5\sigma,\tilde{\mu}+5\sigma\right]$. As we
saw before, conditioning $\theta$ on a value of $D(i)$ is approximately
equivalent to fixing $\mu$: the number of outliers is going to be the same no
matter what (0 with high probability). However, if we first condition $\theta$ on
$D(i)=a$, and then change this record into $b$, we can choose $b$ so that this
record becomes an outlier; and make it 1 with high probability. Thus, this
mechanism is NP but not DDP\@.


\section{Proof of Proposition~\ref{prop:axioms}}\label{proof:axioms}

For APK-DP, the reformulation of the definition using classical
$\epsdel$-indistinguishability makes the result straightforward: the proof is
the same as for $\epsdel$-DP\@. For PPK-DP, we first reformulate the definition
using $f$-divergence. Let $f(x)=\max(0,1-e^\eps x)$. Then a mechanism $\mecha$
is $\Thepsdel$-PPK-DP iff:
\begin{align*}
\sum_{\hatB} \probac{\hatB}{D(i)=a} D_f\left(O_{a,\hatB}\|O_{b,\hatB}\right) \le \del
\end{align*}
where $O_{x,\hatB}=\mech{D}\cond{\theta,D(i)=x,\hatB}$. This view allows us to
use the monotonicity and joint convexity properties of the $f$-divergence to
immediately prove the result for PPK-DP\@.


\section{Proof of Proposition~\ref{prop:more-knowledge}}\label{proof:more-knowledge}

  Suppose that $\mecha$ is $\left(\Theta_1,\eps\right)$-NP\@. For a distribution
  $\theta_2\in\Theta_2$ and an index $i$, let $\theta_1\in\Theta_1$ be such that
  $\theta_1$ is stronger than $\theta_2$. By definition, there exists an
  acceptable normalization $\hatheta\left(\phi_0,\dots,\phi_k\right)$ common to
  $\theta_1$ and $\theta_2$. Let $f$ be the function extracting the sensitive
  value from $\phi_0$ in this normalization. Denoting $I_1$ and $I_2$ the set of
  parameters corresponding respectively to $\theta_1$ and $\theta_2$, as a
  simplification, we assume that $I_2 = \varnothing$ and $I_1 = \{1\}$; it is
  straightforward to adapt the proof to the more generic case. For any output
  $O$, and all values $a,b\in\tuples$, we can decompose:
  \begin{align*}
    & \probac{\mech{D}=O}{f(\phi_0)=a} \\
    & \hs  = \sum_{\hatB} \probac{\phi_1=\hatB}{f(\phi_0)=a} \\
    & \hhs \cdot \probac{\mech{D}=O}{f(\phi_0)=a,\phi_1=\hatB}.
  \end{align*}
  The $\phi_i$ are independent: $\probac{\phi_1=\hatB}{f(\phi_0)=a}$ is
  the same as $\probac{\phi_1=\hatB}{f(\phi_0)=b}$. Since $\mecha$ satisfies
  $\left(\Theta_1,\eps\right)$-NP, we also have for all $\hatB$:
  \begin{align*}
    & \probac{\mech{D}=O}{f(\phi_0)=a,\phi_1=\hatB} \\
    & \hs \le e^\eps\probac{\mech{D}=O}{f(\phi_0)=b,\phi_1=\hatB}.
  \end{align*}
  Thus:
  \begin{align*}
    & \probac{\mech{D}=O}{f(\phi_0)=a} \\
      & \hs \le e^\eps \sum_{\hatB} \probac{\phi_1=\hatB}{f(\phi_0)=b} \\
      & \hhs \cdot \probac{\mech{D}=O}{f(\phi_0)=b\wedge\phi_1=\hatB} \\
      & \hs \le e^\eps \probac{\mech{D}=O}{f(\phi_0)=b} 
  \end{align*}
  and thus, $\mecha$ satisfies $\left(\Theta_2,\eps\right)$-NP\@.
  Adapting the proof to cases where $I_1 \subseteq I_2$ is straightforward.


\section{Proof of Theorem~\ref{thm:apk-ppk}}\label{proof:apk-ppk}

We decompose $\PPK_{i,a,b}$ depending the value of $B$.
\begin{align*}
& \PPK_{i,a,b} \\
& \; = \sum_{\hatD,\hatB}\probac{\dhd,\hatB}{D(i)=a}\expectu{O\sim\mech{\hatD}}{\mohb} \\
& \; = \sum_{\hatB}\probac{\hatB}{D(i)=a}\sum_{\hatD}\probac{\dhd}{D(i)=a,\hatB}\\
  & \hhs \hhs \cdot \expectu{O\sim\mech{\hatD}}{\mohb} \\
& \; = \sum_{\hatB}\probac{\hatB}{D(i)=a}\expectu{\theta\cond{D(i)=a,\hatB},O\sim\mech{D}}{\mohb} \\
& \; = \sum_{\hatB}\probac{\hatB}{D(i)=a}\APK_{i,a,b,\hatB} \\
& \; = \expectu{\theta\cond{D(i)=a}}{APK_{i,a,b,B}}.
\end{align*}

For the second part of the statement, if the mechanism is $\epsdel$-APK-DP, then
for all $i$, $a$, $b$, and $\hatB$, $\APK_{i,a,b,\hatB}\le\del$, so:
\begin{align*}
  \PPK_{i,a,b} = \expectu{\theta\cond{D(i)=a}}{\APK_{i,a,b,B}} \le \del
  %\\
  %& \le \expectu{\theta\cond{D(i)=a}}{\del}\\
  %& \le \del.
\end{align*}

For the last part of the statement, assume that $\mecha$ is $\Theps$-PPK-DP\@.
Then:
\begin{align*}
0 = \PPK_{i,a,b} = & \expectu{\theta\cond{D(i)=a}}{\APK_{i,a,b,B}}.
\end{align*}
All summands are nonnegative, so the sum can only be $0$ if all summands are
$0$: for all $\hatB$, $\APK_{i,a,b,\hatB}=0$, and $\mecha$ is $\Theps$-APK-DP\@.


\section{Proof of Theorem~\ref{thm:apk-ppk-reducible}}\label{proof:apk-ppk-reducible}

First, we prove a technical lemma on the consequences of $\Theta$-reducibility
on the PLRV under $B_1$ and $B_2$.

\begin{lemma}\label{lem:theta-reducibility-plrv}
Let $\Theta$ be a family of distributions, and $\mecha$ a $\Theta$-reducible.
Then, for all $O\in\outputs$ and all $B_1,B_2\in\knowledges$:
\begin{equation*}
  \privlossMit{a}{b}(O,B_1)= \privlossMit{a}{b}(\phi_{B_1,B_2}(O),B_2).
\end{equation*}
\end{lemma}

This statement directly follows by unfolding the definition of
$\privlossMit{a}{b}(O,B_1)$ (Definition~\ref{def:plrv-pk}) and
$\Theta$-reducibility (Definition~\ref{def:theta-reducibility}):
\begin{align*}
  & \privlossMit{a}{b}(O,B_1) \\
  & \; = \ln\frac{\probasc{\theta}{\mech{D}=O}{D(i)=a,B=B_1}}%
                 {\probasc{\theta}{\mech{D}=O}{D(i)=b,B=B_1}} \\
  & \; = \ln\frac{\probasc{\theta}{\mech{D}=\phi_{B_1,B_2}(O)}{D(i)=a,B=B_2}}
                 {\probasc{\theta}{\mech{D}=\phi_{B_1,B_2}(O)}{D(i)=b,B=B_2}} \\
  & \; = \privlossMit{a}{b}(\phi_{B_1,B_2}(O),B_2)
\end{align*}

We can now prove Theorem~\ref{thm:apk-ppk-reducible}. We only need to prove the
reverse implication. Recall that
$m\left(O,B\right)=\max\left(0,1-e^{\eps-\privlossMit{a}{b}(O,B)}\right)$, and
fix $B_0\in\knowledges$. Abusing notations, we denote $B_0$ (resp. $\hatB$) the
event ``$B=B_0$'' (resp. $B=\hatB$), $\hatD$ the event ``$D=\hatD$'', and $a$
the event ``$D(i)=a$''. We have:
\begin{align*}
& \PPK_{i,a,b} \\
& \; = \sum_{\hatD}\probac{\hatD}{a} \sum_{\hatB}\probac{\hatB}{a,\hatD}\\
& \qquad \sum_{\hatO}\probac{\mech{D}=\hatO}{a,\hatB,\hatD} m\left(\hatO,\hatB\right)\\
%
\intertext{Now, we can apply Definition~\ref{def:theta-reducibility} and
Lemma~\ref{lem:theta-reducibility-plrv}, which gives:}
%
& \; = \sum_{\hatD}\probac{\hatD}{a} \sum_{\hatB}\probac{\hatB}{a,\hatD}\\
& \qquad \sum_{\hatO} \probac{\mech{D}=\phi_{\hatB,B_0,i}(\hatO)}{a,B_0,\hatD}\\
& \qquad \qquad m\left(\phi_{\hatB,B_0,i}(\hatO),B_0\right).
%
\intertext{As $\phi_{\hatB,B_0,i}$ is bijective, we can simply rename the $\hatO$:}
%
& \; = \sum_{\hatD}\probac{\hatD}{a} \sum_{\hatB}\probac{\hatB}{a,\hatD}\\
& \qquad \sum_{\hatO} \probac{\mech{D}=\hatO}{a,B_0,\hatD} m\left(\hatO,B_0\right)
%
\intertext{As the last sum does not depend on $\hatB$ anymore, we can reorder
the sums (using distributivity):}
%
& = \sum_{\hatD}\probac{\hatD}{a} \sum_{\hatO} \probac{\mech{D}=\hatO}{a,B_0,\hatD} \\
&  \qquad m\left(\hatO,B_0\right) \underbrace{\sum_{\hatB}\probac{\hatB}{a,\hatD}}_{=1}\\
%
& = \APK_{i,a,b,B_0}.\\
\end{align*}


\section{Proof of Proposition~\ref{prop:reducible-mechanisms}}\label{proof:reducible-mechanisms}

Fix $\tit$. For counting queries, given $B_1,B_2\in\knowledges$, define
$\phi_{B_1,B_2,i}^{count}(\mech{D})=\mech{D}-\mech{B_1}+\mech{B_2}$. This
function is linear, so injective. Call $\theta'$ the random distribution of the
$n-k$ records not present in $B$. Then for all $a\in\tuples$ and all
$O\in\outputs$:
\begin{align*}
  & \probasc{\theta}{\mech{D}=O}{D(i)=a,B=B_1} \\
  & \; = \probasc{D'\sim\theta'}{\mech{D' \cup B_1}=O}{{(D'\cup B_1)}_i=a} \\
  & \; =\probasc{D'\sim\theta'}{\mech{D' \cup B_2}=\phi_{B_1,B_2,i}^{count}(O)}{{(D'\cup B_2)}_i=a} \\
  & \; =\probasc{\theta}{\mech{D}=\phi_{B_1,B_2,i}^{count}(O)}{D(i)=a,B=B_2}.
\end{align*}

For linear queries, we use a similar mapping to $\phi$, which also depends on
the mapping. Let $I$ be the indices of records present in $B$; then a linear
query is $\Theta$-reducible with
\begin{align*}
  \phi_{B_1,B_2,i}^{linear}(\mech{D})
    = \mech{D}+\sum_{j\in I} \alpha_j\left({\left(B_2\right)}_j-{\left(B_1\right)}_j\right).
\end{align*}
This also proves the result for the arithmetic mean.

Similarly, it is easy to verify that the following $\phi$ functions show
$\Theta$-reducibility for the geometric, harmonic and quadractic mean.
\begin{align*}
 & \phi_{B_1,B_2,i}^{geometric}(\mech{D})
    = {\left(\mech{D}^n\cdot\frac{\prod_{j\in I}{\left(B_2\right)}_j}{\prod_{j\in I}{\left(B_1\right)}_j}\right)}^{1/n} \\
 & \phi_{B_1,B_2,i}^{harmonic}(\mech{D}) \\
 & \hs = n{\left({\left(\frac{\mech{D}}{n}\right)}^{-1}
     + \sum_{j}\left(\frac{1}{{\left(B_2\right)}_j}-\frac{1}{{\left(B_1\right)}_j}\right)\right)}^{-1} \\
 & \phi_{B_1,B_2,i}^{quadratic}(\mech{D}) \\
 & \hs = \sqrt{n\cdot\mech{D}^2 + \sum_j\frac{{\left(B_2\right)}_j^2-{\left(B_1\right)}_j^2}{n}}
\end{align*}
The injectivity of each of these functions is clear.


\section{Proof of Theorem~\ref{thm:binary-voting}}\label{proof:binary-voting}

Let us formalize the first intuition. A Bernoulli trial of probability $p_i$
(denoted $\ber{p_i}$), with $\lambda<p_i<1-\lambda$, can be decomposed into the
following process:
\begin{itemize}
\item Generate $b\sim\ber{2\lambda}$.
\item If $b=0$, return $b_{\nu_i}\sim\ber{\frac{p_i-\lambda}{1-2\lambda}}$.
\item If $b=1$, return $b_{rr}\sim\ber{0.5}$.
\end{itemize}
This can be seen as a \emph{randomized response} process applied on some input
$b_{\nu_i}$, itself random: $\theta=\rrdl(\nu)$, where $\nu$ is a distribution
generating $n$ records, where the $i$-th record is generated by
$b_{\nu_i}\sim\ber{\frac{p_i-\lambda}{1-2\lambda}}$, and $\rrdl$ is a binary
randomized response process with parameter $2\lambda$.

Further, note that $\mecha$ can be seen as the composition between itself and a
pre-shuffling phase: $\mecha=\mecha\circ\shuffle$, where
$\shuffle:\datasets\rightarrow\datasets$ is a function that applies a random
permutation to the input records. Thus,
$\mech{D}\cond{D\sim\theta}=\mech{\shuffl{\rrdl(D)}}\cond{D\sim\nu}$. We can
now apply Theorem~3.1 in~\cite{balle2019privacy} to show that
$\shuffle\circ\rrdl$ is $\epsdel$-DP for $\eps$ within the constraints above
(with $k=2$ and $\gamma=2\lambda$). By post-processing,
$\mecha\circ\shuffle\circ\rrdl$ is also $\epsdel$-DP, which directly yields that
$\mecha$ is $\epsdel$-APK-DP\@.

Note that we omitted a small technical detail: conditioning $\theta$ on $D(i)=a$
is not identical to conditioning $\nu$ on $D(i)=a$, since no noise is
added to the record $i$ in the former case. To fix this, we need to define
$\rrdl$ as randomizing all records except a fixed one $i$. The proof of
Theorem~3.1 in~\cite{balle2019privacy} assumes that no noise is added to the
target record, so the result still holds.


\section{Proof of Theorem~\ref{thm:thresholding}}\label{proof:thresholding}

First, let us compute the PLRV for $\mecha_T$ depending on the output $k$ and
the value of the background knowledge $B$, assuming a simple distribution
$\theta$ where records are i.i.d. Denote by $b$ the number of records in $B$
which are 1 and by $\ol{b}=|B|-b$ the number of records that are 0. The targeted
record will be called $D(t)$, and we assume it is never part of $B$.

\begin{calc}[PLRV for thresholding]\label{ratio}
Let $\theta$ be a distribution that returns $n$ i.i.d records according to
$D(i)\sim Ber(p)$. Then the value of
$\privlossit{0}{1}{\mecha_T}(k,B) =
    \ln \left(\frac{\probac{\mech{D}=k}{D(t)=0,\zeta(D)=B}}{\probac{\mech{D}=k}{D(t)=1,\zeta(D)=B}} \right)$
is given by:
\begin{itemize}
  \item $\ln\frac
    {\sum_{s=0}^{T-b} p^s {(1-p)}^{n-|B|-1-s} \binom{n-|B|-1}{s}}
    {\sum_{s=0}^{T-b-1} p^s {(1-p)}^{n-|B|-1-s} \binom{n-|B|-1}{s}}$ 
    if $k=\bot$;
  \item $\ln\frac{p(n-\ol{b}-k)}{(1-p)(k-b)}$ otherwise.
\end{itemize}

Note that if $k=b$, then $\privlossit{0}{1}{\mecha_T}(k,B)=\infty$. The case
where $k<b$ is impossible regardless of $D(i)$ (there cannot be more $1$s in the
background knowledge than the mechanism outputs).

In the case where there is no background knowledge, this becomes:
\begin{itemize}
  \item $\ln\frac
    {\sum_{s=0}^{T} p^s {(1-p)}^{n-1-s} \binom{n-1}{s}}
    {\sum_{s=0}^{T-1} p^s {(1-p)}^{n-1-s} \binom{n-1}{s}}$ if $k=\bot$;
  \item $\ln\frac{p(n-k)}{(1-p)k}$ otherwise.
\end{itemize}
\end{calc}

This calculation allows us to deduce the $\epsdel$ parameters in the simpler
case where there is no background knowledge. To do so, we need a technical
lemma on the estimation of sums appearing in the formula above.

\begin{lemma}\label{lem:partial-binomial}
\begin{align*}
\sum_{s=0}^T f(s,n,p) > 1-\frac{C}{C-1} f(T+1,n,p).
\end{align*}

\begin{proof}
We can rewrite
\begin{align*}
\sum_{s=0}^T f(s,n,p) = 1-\sum_{s=T+1}^n f(s,n,p).
\end{align*}
Now, note that
\begin{align*}
\frac{f(s,n,p)}{f(s-1,n,p)} = \frac{p}{1-p}\left(\frac{n-s+1}{s}\right) \le \frac{pn}{(1-p)s}.
\end{align*}
  For $s > T = \frac{Cnp}{1-p}$, this is smaller than $1/C$, so the sum
converges at least as fast as a geometric series, which gives
\begin{align*}
\sum_{s=T+1}^n f(s,n,p) < \frac{C}{C-1} f(T+1,n,p).
\end{align*}
\end{proof}
\end{lemma}

We can now start proving the main theorem; first in the case where there is no
background knowledge and all $p_i$ are equal. There are two possibilities to
consider, $\privlossit{1}{0}{\mecha_T}$ and $\privlossit{0}{1}{\mecha_T}$.
First, we have:
\begin{align*}
& \probasc{\theta}{\mecha_T(D)\neq\bot}{D(i)=0} \\
  & \quad < \probasc{\theta}{\mecha_T(D)\neq\bot}{D(i)=1} \\
  & \quad = 1 - \sum_{s=0}^{T-1} f(s,n-1,p) \\
  & \quad < \frac{C}{C-1} f(T,n-1,p),
\end{align*}
so we will denote this quantity as $\del$. Now, we have
\begin{align*}
\privlossit{1}{0}{\mecha_T}(\bot)
  =\ln\frac
    {\sum_{s=0}^{T-1} f(s,n-1,p)}
    {\sum_{s=0}^{T} f(s,n-1,p)}
  < 0.
\end{align*}
Furthermore
\begin{align*}
\privlossit{0}{1}{\mecha_T}(\bot)
  & = \ln\frac
    {\sum_{s=0}^{T} f(s,n-1,p)}
    {\sum_{s=0}^{T-1} f(s,n-1,p)} \\
  & < \ln\left(\frac
    {1}
    {1-\frac{C}{C-1}f(T,n-1,p)}\right) \\
  & = -\ln\left(1-\frac{C}{C-1}f(T,n-1,p)\right).
\end{align*}
Thus, when the output was thresholded, the PLRV is smaller than
$\eps=-\ln\left(1-\frac{C}{C-1}f(T,n-1,p)\right)$ and the event ``the output is
not thresholded'' only happens with a probability smaller than $\del$, which
proves the initial statement in the simpler case.

Now, in the case where the background knowledge is non-empty, we must not only
split the output space, but also $\mathcal{B}$ as well. Most of the probability
mass will be in the event where the output is thresholded and the background
knowledge has very few ``1'' entries. This means that if $b$ denotes the number
of ``1'' entries in $B$, we split $\mathcal{B}$ in the background knowledges
with $b < b_{\max}$ and those with $b\ge b_{\max}$. Again, we calculate the
$\eps$ for this event and put the other events in $\del$.
\begin{align*}
& \probasc{\theta}{b \ge b_{\max} \vee \mecha_T(D)\neq\bot}{D(i)=0} \\
  & < \probas{\theta}{b \ge b_{\max}} + \probasc{\theta}{\mecha_T(D)\neq\bot}{b \ge b_{\max}, D(i)=1} \\
  & < (1 - \sum_{s=0}^{b_{\max}-1} f(s,|B|,p)) + (1 - \sum_{s=0}^{T'-1} f(s,n-|B|-1,p)) \\
  & < \frac{C_b}{C_b-1} f(b_{\max},|B|,p) + \frac{C'}{C'-1} f(T',n-|B|-1,p)
\end{align*}
and we denote this quantity as $\del$. Let $\hatB$ be a background knowledge
  with $b < b_{\max}$. We have
\begin{align*}
\privlossit{1}{0}{\mecha_T}(\bot,\hatB)
  =\ln\frac
    {\sum_{s=0}^{T-b-1} f(s,n-|B|-1,p)}
    {\sum_{s=0}^{T-b} f(s,n-|B|-1,p)}
  < 0.
\end{align*}
Moreover:
\begin{align*}
& \privlossit{0}{1}{\mecha_T}(\bot,\hatB) \\
  & \quad = \ln\frac
    {\sum_{s=0}^{T-b} f(s,n-|B|-1,p)}
    {\sum_{s=0}^{T-b-1} f(s,n-|B|-1,p)} \\
  & \quad < \ln\left(\frac
    {1}
    {\sum_{s=0}^{T'-1} f(s,n-|B|-1,p)}\right) \\
  & \quad < -\ln\left(1 - \frac{C'}{C'-1} f(T',n-|B|-1,p)\right) 
\end{align*}
Thus, when the output was thresholded and the ``1''s in the background knowledge
are bounded by $b_{\max}$, the PLRV is smaller than
$\eps=-\ln\left(1-\frac{C'}{C'-1} f(T',n-|B|-1,p) \right)$ and complementary
event only happens with probability smaller than $\del$.

Now, we extend the first case (where the background knowledge is empty) to the
case where all $p_i$ are different, and $p_i<p$ for all $p$. Let us denote
$\theta_p$ the distribution where all users vote with the same probability $p$.
Let $g(s,n,p)=\probas{\theta}{\mecha_T(D)=s}$. By a simple coupling argument
between $\theta$ and $\theta_p$, we have for all $t$:
\begin{align*}
\sum_{s=t+1}^n g(s,n,p)
  & = \probas{\theta}{\mecha_T(D)>t} \\
  & \le \probas{\theta_p}{\mecha_T(D)>t} \\
  & = \sum_{s=t+1}^n f(s,n,p).
\end{align*}
We can then use this fact throughout the previous proof. The application of this
bound for $\del$ is immediate, and for $\eps$, we have:
\begin{align*}
\privlossit{0}{1}{\mecha_T}(\bot,\hatB)
  & = \ln\frac
    {\sum_{s=0}^{T} g(s,n-1,p)}
    {\sum_{s=0}^{T-1} g(s,n-1,p)}.
\end{align*}
We can bound the numerator by $1$ and the denominator expands to:
\begin{align*}
\sum_{s=0}^{T-1} g(s,n-1,p)
  & = 1 - \sum_{s=T}^{n-1} g(s,n-1,p) \\
  & \ge 1 - \sum_{s=T}^{n-1} f(s,n-1,p) \\
  & = \sum_{s=0}^{T-1} f(s,n-1,p)
\end{align*}
so we can reuse the previous bound. The bounds translate to the case where the
background knowledge is not empty by a similar argument.


\section{Proof sketch of Proposition~\ref{prop:thresholding-apk-partial}}\label{proof:thresholding-apk-partial}

By writing down its explicit value, one can see that $\APK_{i,a,b,B}$, with $a,b
\in \{0,1\}$, only depends on the difference between $T$ and the number of ones
$b$ in the background knowledge $B$. The same applies for the variables $n$ and
$|B|$, which appear only in the form of $n-|B|$. This shows the equivalence of
$\mecha_T$ being $(\{\theta\},\eps,\del)$-APK-DP and $\mecha_{T-|B|}$ being
$(\{\theta'\},\eps,\del)$-APK-DP\@. Since APK-DP and PPK-DP are the same when
there is no background knowledge, the statement follows.

\begin{comment}
\begin{align*}
&\APK_{t,0,1,B} \\
&=\sum_{\hatD} \probac{D=\hatD}{D_t = 0, \zeta(D)=\hatB} \cdot m(\mecha(\hatD),\hatB) \\
&=
\sum_{k =b+1}^{\min(T,n-(|B|-b)-1)} p^{k-b} (1-p)^{n-(|B|-b)-k-1}  \binom{n-|B|-1}{k-b} \\
&\cdot \max \left( 0,1-e^{\epsilon-\ln \left( \frac{\sum_{s=0}^{T-b} (\frac{p}{1-p})^s \binom{n-|B|-1}{s}}{\sum_{s=0}^{T-b-1}(\frac{p}{1-p})^s \binom{n-|B|-1}{s}} \right) }\right)  \\
&+ \sum_{k= \max (b+1, T+1) }^{n-(|B|-b)-1} p^{k-b} (1-p)^{n-(|B|-b)-k-1} \binom{n-|B|-1}{k-b} \\
&\cdot \max \left( 0,1-e^{\epsilon-\ln \left( \frac{(p) (n-(|B|-b)-k)}{(1-p) (k-b)} \right) } \right) 
+  (1-p)^{n-|B|-1} \\
&=
\sum_{k =1}^{\min(T-b,n-|B|-1)} p^{k} (1-p)^{n-|B|-k-1}  \binom{n-|B|-1}{k} \\
&\cdot \max \left( 0,1-e^{\epsilon-\ln \left( \frac{\sum_{s=0}^{T-b} (\frac{p}{1-p})^s \binom{n-|B|-1}{s}}{\sum_{s=0}^{T-b-1}(\frac{p}{1-p})^s \binom{n-|B|-1}{s}} \right) }\right)  \\
&+ \sum_{k= \max (1, T-b+1) }^{n-|B|-1} p^{k} (1-p)^{n-|B|-k-1} \binom{n-|B|-1}{k} \\
&\cdot \max \left( 0,1-e^{\epsilon-\ln \left( \frac{(p) (n-|B|-k)}{(1-p) (k)} \right) } \right) 
+  (1-p)^{n-|B|-1}
\end{align*}
$\APK_{i,1,0,B}$ analogously.
\end{comment}


\section{Proof of Theorem~\ref{thm:sequential-composition}}\label{proof:sequential-composition}

Fix $i$, $a$, $b$, $O$ and $\hatB$. The main statement is straightforward to
prove by decomposing:

\begin{align*}
& \privlossMit{a}{b}(O,\hatB)\\
& \; = \ln\frac{%
    \probasc{\theta}{\mecha(D) = (O_1,O_2)}{D(i)=a, \hatB}
  }{%
    \probasc{\theta}{\mecha(D) = (O_1,O_2)}{D(i)=b, \hatB}
  } \\
%= & \ln\frac{%
%\probasc{\theta}{\mecha_1(D) = O_1, \mecha_2(D) = O_2}{D(i)=a, \hatB}}{%
%\probasc{\theta}{\mecha_1(D) = O_1, \mecha_2(D) = O_2}{D(i)=b, \hatB}} \\
& \; = \ln\frac{%
\probasc{\theta}{\mecha_2(D) = O_2}{\mecha_1(D) = O_1, D(i)=a , \hatB}}{%
\probasc{\theta}{\mecha_2(D) = O_2}{\mecha_1(D) = O_1, D(i)=b, \hatB}}\\
& \; \; + \ln\frac{%
\probasc{\theta}{\mecha_1(D) = O_1}{D(i)=a, \hatB}}{%
\probasc{\theta}{\mecha_1(D) = O_1}{D(i)=b, \hatB}}
\end{align*}

and plugging in the definition of $\Depab$.

%\intertext{Applying plugging the dependency leads to:}
%= & {\Depab}\\
%& + \ln\frac{%
%\probasc{\theta}{\mecha_1(D) = O_1}{D(i)=a, \hatB}}{%
%\probasc{\theta}{\mecha_1(D) = O_1}{D(i)=b, \hatB}}\\
%&+\ln\frac{%
%\probasc{\theta}{\mecha_2(D) = O_2}{D(i)=a, \hatB}}{%
%\probasc{\theta}{\mecha_2(D) = O_2}{D(i)=b, \hatB}} \\
%= & \Depab\\
%& +\privlossit{a}{b}{\mecha_1}(O_1,\hatB)+\privlossit{a}{b}{\mecha_2}(O_2,\hatB).

To prove the composition theorem, we have to show that, if we denote
$\eps=\eps_1+\eps_2+\mu$ and $\del=\del_1+\del_2+\nu$:
\begin{align*}
  \expectu{\theta\cond{D(i)=a,\hatB},O\sim\mech{D}}{\max\left(0,1-e^{\eps-\privlossMit{a}{b}(O,\hatB)}\right)}\le\del.
\end{align*}
Note that the function $f(x)=\max\left(0,1-e^x\right)$ is subadditive: for all $x$
and $y$, $f(x+y)\le f(x)+f(y)$. Indeed, if $x>0$, then $f(x)=0$, and it is
straightforward to verify that $1-e^{x+y}\le1-e^y$. The same reasoning holds
when $y>0$. Finally, if $x\le0$ and $y\le0$, then we must show that
$1-e^{x+y}\le2-e^x-e^y$, which is equivalent to
$\left(e^x-1\right)\left(e^y-1\right)\ge0$, which trivially holds.

We then define $a=\eps_1-\privlossit{a}{b}{\mecha_1}\left(O_1,\hatB\right)$,
$b=\eps_2-\privlossit{a}{b}{\mecha_2}\left(O_2,\hatB\right)$, and
$c=\mu-\Depab$, and we use this subadditivity property: $f(a+b+c)\le
f(a)+f(b)+f(c)$. As we have
$a+b+c=\eps-\privlossit{a}{b}{\mecha}\left(O,\hatB\right)$, we can directly plug
this into the expression above and use the assumptions of the theorem to show
that it is bounded by $\del_1+\del_2+\nu=\del$.

